Star formation at high redshift as traced by near-infrared Halpha surveys

Surveys of redshifted emission lines in the near-infrared will provide unique information on the cosmic star formation history. Near-infrared Halpha surveys will probe the cosmic star formation density and the evolution of the luminosity function of star forming galaxies out to z\sim2.5, including the important z=1.5-2.0 epoch, where according to current knowledge the cosmic star formation density peaks. Halpha and other hydrogen recombination lines (except Lyman alpha) and [O II] are all useful tracers of star formation provided the luminosity function is probed to sufficiently deep levels. However, shallow surveys or surveys of Lyman alpha or [O III] emission are not suitable for measuring or even constraining the cosmic star formation density. A first estimate of the star formation density at z\approx2.25 is derived, based on a new and sensitive large-area ESO near-infrared survey for Halpha emission at this redshift. Future observational directions, at near-infrared and longer wavelengths, for reading the cosmic star formation history are outlined.

==> hyphens.tex <==
\hyphenation{ASTRON}                    % how to (not) break these words
\hyphenation{cloud-let cloud-lets}
\hyphenation{HVABG}
\hyphenation{MNRAS}
\hyphenation{Peim-bert}
\hyphenation{Schloerb}
\endinput


==> molec.tex <==
%--------------- molecules and molecular ions --------------------------------
%

\def\mbox{\hbox}           % for compatibility of TeX and LaTeX use 

\def\CO#1{\ifnum#1=0                    % CO isotopes
           \ifmmode \mbox{\rm CO}
           \else {\rm CO}
           \fi
          \else
           \ifnum#1<15
            \ifmmode ^{#1}\mbox{\rm CO}
            \else $^{#1}${\rm CO}
            \fi
           \else
            \ifmmode \mbox{\rm C}^{#1}\mbox{\rm O}
            \else {\rm C}$^{#1}${\rm O}
            \fi
           \fi
          \fi}

\def\COp{\ifmmode \mbox{\rm CO}^+           %   +
         \else {\rm CO}$^+$                 % CO
         \fi}

\def\CS#1{\ifnum#1=0                    % CS isotopes
           \ifmmode \mbox{\rm CS}
           \else {\rm CS}
           \fi
          \else
           \ifnum#1<15
            \ifmmode ^{#1}\mbox{\rm CS}
            \else $^{#1}${\rm CS}
            \fi
           \else
            \ifmmode \mbox{\rm C}^{#1}\mbox{\rm S}
            \else {\rm C}$^{#1}${\rm S}
            \fi
           \fi
          \fi}

\def\HCOp{\ifmmode \mbox{\rm HCO}^+          %    +
          \else {\rm HCO}$^+$                % HCO
          \fi}
                                               %  +
\def\Hthreep{\ifmmode \mbox{\rm H}_3^+         % H
             \else {\rm H}$_3^+$               %  3
             \fi}

\def\Htwo{\ifmmode \mbox{\rm H}_2              % H
          \else {\rm H}$_2$                    %  2
          \fi}

\def\HtwoO{\ifmmode \mbox{\rm H}_2\mbox{\rm O} % H O
           \else {\rm H}$_2${\rm O}            %  2
           \fi}

%
%---------------------- atoms and atomic ions ---------------------------------
%

\def\ion#1#2{\ifmmode \mbox{{\rm #1}}\,\mbox{{\sc #2}} % generic ion
        \else {\rm #1}$\,${\sc #2}
        \fi}
\def\HI{\ion{H}{i}}
\def\HII{\ion{H}{ii}}

%
%-------------------- hydrogen recombination lines ---------------------------
%

\def\rec#1#2{\if#2a                            % generic
              \ifmmode \mbox{{\rm #1}}\alpha   % recombination line
              \else {\rm #1}$\alpha$
              \fi
             \fi
             \if#2b
              \ifmmode \mbox{{\rm #1}}\beta
              \else {\rm #1}$\beta$
              \fi
             \fi
             \if#2g
              \ifmmode \mbox{{\rm #1}}\gamma
              \else {\rm #1}$\gamma$
              \fi
             \fi}

\def\Lya{\rec{Ly}{a}}                          % Lyman alpha
\def\Ha{\rec{H}{a}}                            % H alpha
\def\Brg{\rec{Br}{g}}                          % Brackett gamma

\endinput


==> refs.tex <==
%..............................................................................
%
%             This is    r e f s . t e x
%
% A LaTeX file for keeping tracks of references to figures, sections,
% tables and equations.
%
% Latest update: Paul van der Werf 21-Mar-1994
%
%..............................................................................

\newcommand{\tabref}[1]{Table~\protect\ref{#1}}
\newcommand{\figref}[1]{Fig.~\protect\ref{#1}}
\newcommand{\figrefbare}[1]{\protect\ref{#1}}
\newcommand{\figrefs}[1]{Figs.~\protect\ref{#1}}
\newcommand{\figsref}[2]{Figs.~\protect\ref{#1}--\protect\ref{#2}}
\newcommand{\twofigsref}[2]{Figs.~\protect\ref{#1} and~\protect\ref{#2}}
\newcommand{\eqref}[1]{Eq.~$\left(\protect\ref{#1}\right)$}
\newcommand{\eqsref}[2]{Eqs.~$\left(\protect\ref{#1}\right)$--$\left(\protect\ref{#2}\right)$}
\newcommand{\secref}[1]{Sect.~\protect\ref{#1}}
\newcommand{\secsref}[2]{Sects.~\protect\ref{#1}--\protect\ref{#2}}
\newcommand{\twosecsref}[2]{Sects.~\protect\ref{#1} and~\protect\ref{#2}}

% upper case versions to begin sentences: 

\newcommand{\Tabref}[1]{\tabref{#1}}
\newcommand{\Figref}[1]{Figure~\protect\ref{#1}}
\newcommand{\Figrefs}[1]{Figures~\protect\refs{#1}}
\newcommand{\Figsref}[2]{Figures~\protect\ref{#1}--\protect\ref{#2}}
\newcommand{\Eqref}[1]{Equation~(\protect\ref{#1})}
\newcommand{\Eqsref}[2]{Equations~(\protect\ref{#1})--(\protect\ref{#2})}
\newcommand{\Secref}[1]{Section~\protect\ref{#1}}

\endinput


==> symbols.tex <==
%------------------ degrees, magnitudes, RA, Dec etc -------------------------
%

\def\deg{\ifmmode ^\circ                % degrees symbol
         \else $^\circ$
         \fi
         \hskip -0.1truecm}
\def\degd#1.#2{                         % degrees over decimal point
                                        % syntax: \degd 4.3 or \degd 4.{34}
               \ifmmode {#1^{\hskip 0.05em\circ}\hskip-0.42em.\hskip0.08em#2}
               \else {#1$^{\hskip 0.05em\circ}\hskip-0.42em.\hskip0.08em$#2}
               \fi
              }
\def\mind#1.#2{                         % minutes over decimal point
                                        % syntax: \mind 4.3
               \ifmmode {#1^{\hskip 0.05em\prime}\hskip-0.35em.\hskip0.05em#2}
               \else {#1$^{\hskip 0.05em\prime}\hskip-0.35em.\hskip0.05em$#2}
               \fi
              }
\def\secd#1.#2{                         % seconds over decimal point
                                        % syntax: \secd 4.3
               \ifmmode {#1^{\prime\prime}\hskip-0.46em.\hskip0.12em#2}
               \else {#1$^{\prime\prime}\hskip-0.46em.\hskip0.12em$#2}
               \fi
              }
\def\timsecd#1.#2{                      % time seconds over decimal point
                                        % syntax: \timsecd 4.3
                  \ifmmode {#1^{\rm s}\hskip-0.39em.\hskip0.08em#2}
                  \else {$#1^{\rm s}\hskip-0.39em.\hskip0.08em#2$}
                  \fi
                 }
\def\hms#1h#2m#3s{                      % hms format (for RA)
                                        % syntax: \hms 12h34m45s
                  \relax
                  \ifmmode #1^{\rm h}\,#2^{\rm m}\,#3^{\rm s}
                  \else \hbox{$#1^{\rm h}\,#2^{\rm m}\,#3^{\rm s}$}
                  \fi
                 }
\def\dms#1d#2m#3s{                      % dms format (for Dec)
                                        % syntax: \dms 12d14m45s
                  \relax
                  \ifmmode #1^\circ\,#2^{\prime}\,#3^{\prime\prime}
                  \else \hbox{$#1^\circ\,#2^{\prime}\,#3^{\prime\prime}$}
                  \fi
                 }
\def\dmsd#1d#2m#3.#4s{                  % dms format with decimal point (Dec)
                                        % syntax: \dmsd 12d13m34.5s
                      \relax
                      \ifmmode #1^\circ\,#2^{\prime}\,#3^{\prime\prime}
                               \hskip-0.46em.\hskip0.12em#4
                      \else \hbox{$#1^\circ\,#2^{\prime}\,#3^{\prime\prime}
                            \hskip-0.46em.\hskip0.12em#4$}
                      \fi
                     }
\def\hm#1h#2m{                          % hm format (for RA)
                                        % syntax: \hm 12h13m
              \relax
              \ifmmode #1^{rm h}\,#2^{\rm m}
              \else \hbox{$#1^{\rm h}\,#2^{\rm m}$}
              \fi
             }
\def\dm#1d#2m{                          % dm format (for Dec)
                                        % syntax: \dm 12d13m
              \relax
              \ifmmode #1^\circ\,#2^{\prime}
              \else \hbox{$#1^\circ\,#2^{\prime}$}
              \fi
             }
\def\hmsd#1h#2m#3.#4s{                  % hms format with decimal point (RA)
                                        % syntax: \hmsd 12h13m34.5s
                      \relax
                      \ifmmode #1^{\rm h}\,#2^{\rm m}\,#3^{\rm s}
                               \hskip-0.39em.\hskip0.08em#4
                      \else \hbox{$#1^{\rm h}\,#2^{\rm m}\,#3^{\rm s}
                            \hskip-0.39em.\hskip0.08em#4$}
                      \fi
                     }
\def\hmd#1h#2.#3m{                  % hm format with decimal point (RA)
                                    % syntax: \hmd 12h13.6m
                  \relax
                  \ifmmode #1^{\rm h}\,#2^{\rm m}
                           \hskip-0.55em.\hskip0.22em#3
                  \else \hbox{$#1^{\rm h}\,#2^{\rm m}
                        \hskip-0.55em.\hskip0.22em#3$}
                  \fi
                 }
\def\mg{\relax                          % magnitudes symbol
        \ifmmode ^{\rm m}
        \else $^{\rm m}$
        \fi
       }
\def\mgd#1.#2{                          % magnitudes over decimal point
                                        % syntax: \mgd 4.3
              \relax
              \ifmmode #1^{\rm m}
                       \hskip-0.55em.\hskip0.22em#2
              \else \hbox{#1$^{\rm m}
                    \hskip-0.55em.\hskip0.22em$#2}
              \fi
             }

%
%-------------------- math symbols --------------------------------------------
%

\def\simlt{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$<$}}}}
\def\simgt{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$>$}}}}

%
%--------------------------- units -------------------------------------------
% use: e.g. $15\kms$
%

\def\unitspace{\,}                      % space to be used with units

\def\un#1{\ifmmode \unitspace{\rm #1} % generic unit
          \else $\unitspace$#1
          \fi}
\def\pun#1#2{\ifmmode \unitspace\mbox{\rm #1}^{#2} % generic unit with a power
             \else $\unitspace$#1$^{#2}$
             \fi}

\def\es{\un{erg}\psec}                %      -1
                                      % erg s
\def\esc{\es\pcmsqu}                  %      -1 -2
                                      % erg s cm
\def\escmum{\esc\mum^{-1}}            %      -1 -2  -1
                                      % erg s cm  mu
\def\escs{\esc\pun{sr}{-1}}           %      -1 -2 -1
                                      % erg s cm sr
\def\escsm{\escs\mum^{-1}}            %      -1 -2 -1 -1
                                      % erg s cm sr mu
\def\GHz{\un{GHz}}                    % GHz
\def\kms{\un{km}\pun{s}{-1}}          %     -1
                                      % km s
\def\Lsun{\ifmmode \un{L}_{\odot}     % solar luminosity
          \else $\un{L}_{\odot}$
          \fi}
\def\Msun{\ifmmode \un{M}_{\odot}     % solar mass
          \else $\un{M}_{\odot}$
          \fi}
\def\mum{\ifmmode \unitspace\mu\mbox{\rm m} % micron
         \else $\unitspace\mu$m
         \fi}
\def\pcmcub{\pun{cm}{-3}}             %   -3
                                      % cm
\def\pcmsqu{\pun{cm}{-2}} %   -2
                          % cm
\def\pyr{\pun{yr}{-1}}    %   -1
                          % yr
\def\psec{\pun{s}{-1}}    %  -1
                          % s

%
%-------------------------- quantities ---------------------------------------
%

\def\Bp{\relax                            % B
        \ifmmode B_{||}                   %  ||
        \else $B_{||}$
        \fi}
\def\Bt{\relax                            % B
        \ifmmode B\!_{\perp}              %  |
        \else $B\!_{\perp}$               %  -
        \fi}
\def\Gcr{\relax                           % Gamma
         \ifmmode \Gamma\!_{\rm cr}       %      cr
         \else $\Gamma\!_{\rm cr}$
         \fi}
\def\ICII{\relax                          % I
          \ifmmode I_{[\CII]}             %  [C II]
          \else $I_{[\CII]}$
          \fi}
\def\LHtwo{\relax                                 % L
           \ifmmode L_{\mbox{\rm\scriptsize H}_2} %  H
           \else $L_{\mbox{\rm\scriptsize H}_2}$  %   2
           \fi}
\def\LLya{\relax                          % L
          \ifmmode L_{{\rm Ly}\,\alpha}   %  Ly alpha
          \else $L_{{\rm Ly}\,\alpha}$
          \fi}
\def\MHtwo{\relax                                 % M
           \ifmmode M_{\mbox{\rm\scriptsize H}_2} %  H
           \else $M_{\mbox{\rm\scriptsize H}_2}$  %   2
           \fi}
\def\MHtwodot{\relax                                       % .
              \ifmmode \dot{M}_{\mbox{\rm\scriptsize H}_2} % M
              \else $\dot{M}_{\mbox{\rm\scriptsize H}_2}$  %  H
              \fi}                                         %   2
\def\Mstardot{\relax                      % .
              \ifmmode \dot{M}_{\ast}     % M
              \else $\dot{M}_{\ast}$      %  *
              \fi}
\def\nHI{\relax                                      % n
         \ifmmode n_{\mbox{\scriptsize\rm H\,\sc I}} %  HI
         \else $n_{\mbox{\scriptsize\rm H\,\sc I}}$
         \fi}
\def\nHtwo{\relax                                % n
           \ifmmode n_{{\mbox{\scriptsize H}}_2} %  H
           \else $n_{{\mbox{\scriptsize H}}_2}$  %   2
           \fi}

%
%------------------ source designations -------------------------
%

\def\sou#1#2{\relax                       % source designations
             \ifmmode {\rm #1}\,{\rm #2}  % e.g. \sou{Arp}{220}
             \else #1$\,$#2
             \fi}

\def\NGC#1{\sou{NGC}{#1}}                % NGC number

%
%------------------- generic quantity symbols ------------------
%

\def\qu#1#2{\relax                          % quantity symbols
            \ifmmode #1_{\rm #2}            % e.g. \qu{L}{FIR}
            \else $#1_{\rm #2}$
            \fi}

\endinput

